Role of Morphogenetic Competency on Evolution

The relationship between intelligence and evolution is bidirectional: while evolution can help evolve intelligences, the degree of intelligence itself can impact evolution (Baldwin, 1896). In the field of Evolutionary Computation, the inverse relationship (impact of intelligence on evolution) is approached from the perspective of organism level behaviour (Hinton, 1996). We extend these ideas to the developmental (cellular morphogenetic) level in the context of an expanded view of intelligence as not only the ability of a system to navigate the three-dimensional world, but also as the ability to navigate other arbitrary spaces (transcriptional, anatomical, physiological, etc.). Here, we specifically focus on the intelligence of a minimal model of a system navigating anatomical morphospace, and assess how the degree and manner of problem solving competency during morphogenesis effects evolutionary dynamics. To this end, we evolve populations of artificial embryos using a standard genetic algorithm in silico. Artificial embryos were cellular collectives given the capacity to undergo morphogenetic rearrangement (e.g., regulative development) prior to selection within an evolutionary cycle. Results from our model indicates that morphogenetic competency significantly alters evolutionary dynamics, with evolution preferring to improve anatomical intelligence rather than perfect the structural genes. These observations hint that evolution in the natural world may be leveraging the problem solving competencies of cells at multiple scales to boost evolvability and robustness to novel conditions. We discuss implications of our results for the Developmental Biology and Artificial Life communities.

==> Chapter1.tex <==
% Chapter 1

\chapter{Introduction} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\begin{comment}
\section{Welcome and Thank You}
Welcome to this \LaTeX{} Thesis Template, a beautiful and easy to use template for writing a thesis using the \LaTeX{} typesetting system.

If you are writing a thesis (or will be in the future) and its subject is technical or mathematical (though it doesn't have to be), then creating it in \LaTeX{} is highly recommended as a way to make sure you can just get down to the essential writing without having to worry over formatting or wasting time arguing with your word processor.

\LaTeX{} is easily able to professionally typeset documents that run to hundreds or thousands of pages long. With simple mark-up commands, it automatically sets out the table of contents, margins, page headers and footers and keeps the formatting consistent and beautiful. One of its main strengths is the way it can easily typeset mathematics, even \emph{heavy} mathematics. Even if those equations are the most horribly twisted and most difficult mathematical problems that can only be solved on a super-computer, you can at least count on \LaTeX{} to make them look stunning.

%----------------------------------------------------------------------------------------

\section{Learning \LaTeX{}}

\LaTeX{} is not a \textsc{wysiwyg} (What You See is What You Get) program, unlike word processors such as Microsoft Word or Apple's Pages. Instead, a document written for \LaTeX{} is actually a simple, plain text file that contains \emph{no formatting}. You tell \LaTeX{} how you want the formatting in the finished document by writing in simple commands amongst the text, for example, if I want to use \emph{italic text for emphasis}, I write the \verb|\emph{text}| command and put the text I want in italics in between the curly braces. This means that \LaTeX{} is a \enquote{mark-up} language, very much like HTML.

\subsection{A (not so short) Introduction to \LaTeX{}}

If you are new to \LaTeX{}, there is a very good eBook -- freely available online as a PDF file -- called, \enquote{The Not So Short Introduction to \LaTeX{}}. The book's title is typically shortened to just \emph{lshort}. You can download the latest version (as it is occasionally updated) from here:
\url{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}

It is also available in several other languages. Find yours from the list on this page: \url{http://www.ctan.org/tex-archive/info/lshort/}

It is recommended to take a little time out to learn how to use \LaTeX{} by creating several, small `test' documents, or having a close look at several templates on:\\ 
\url{http://www.LaTeXTemplates.com}\\ 
Making the effort now means you're not stuck learning the system when what you \emph{really} need to be doing is writing your thesis.

\subsection{A Short Math Guide for \LaTeX{}}

If you are writing a technical or mathematical thesis, then you may want to read the document by the AMS (American Mathematical Society) called, \enquote{A Short Math Guide for \LaTeX{}}. It can be found online here:
\url{http://www.ams.org/tex/amslatex.html}
under the \enquote{Additional Documentation} section towards the bottom of the page.

\subsection{Common \LaTeX{} Math Symbols}
There are a multitude of mathematical symbols available for \LaTeX{} and it would take a great effort to learn the commands for them all. The most common ones you are likely to use are shown on this page:
\url{http://www.sunilpatel.co.uk/latex-type/latex-math-symbols/}

You can use this page as a reference or crib sheet, the symbols are rendered as large, high quality images so you can quickly find the \LaTeX{} command for the symbol you need.

\subsection{\LaTeX{} on a Mac}
 
The \LaTeX{} distribution is available for many systems including Windows, Linux and Mac OS X. The package for OS X is called MacTeX and it contains all the applications you need -- bundled together and pre-customized -- for a fully working \LaTeX{} environment and work flow.
 
MacTeX includes a custom dedicated \LaTeX{} editor called TeXShop for writing your `\file{.tex}' files and BibDesk: a program to manage your references and create your bibliography section just as easily as managing songs and creating playlists in iTunes.

%----------------------------------------------------------------------------------------

\section{Getting Started with this Template}

If you are familiar with \LaTeX{}, then you should explore the directory structure of the template and then proceed to place your own information into the \emph{THESIS INFORMATION} block of the \file{main.tex} file. You can then modify the rest of this file to your unique specifications based on your degree/university. Section \ref{FillingFile} on page \pageref{FillingFile} will help you do this. Make sure you also read section \ref{ThesisConventions} about thesis conventions to get the most out of this template.

If you are new to \LaTeX{} it is recommended that you carry on reading through the rest of the information in this document.

Before you begin using this template you should ensure that its style complies with the thesis style guidelines imposed by your institution. In most cases this template style and layout will be suitable. If it is not, it may only require a small change to bring the template in line with your institution's recommendations. These modifications will need to be done on the \file{MastersDoctoralThesis.cls} file.

\subsection{About this Template}

This \LaTeX{} Thesis Template is originally based and created around a \LaTeX{} style file created by Steve R.\ Gunn from the University of Southampton (UK), department of Electronics and Computer Science. You can find his original thesis style file at his site, here:
\url{http://www.ecs.soton.ac.uk/~srg/softwaretools/document/templates/}

Steve's \file{ecsthesis.cls} was then taken by Sunil Patel who modified it by creating a skeleton framework and folder structure to place the thesis files in. The resulting template can be found on Sunil's site here:
\url{http://www.sunilpatel.co.uk/thesis-template}

Sunil's template was made available through \url{http://www.LaTeXTemplates.com} where it was modified many times based on user requests and questions. Version 2.0 and onwards of this template represents a major modification to Sunil's template and is, in fact, hardly recognisable. The work to make version 2.0 possible was carried out by \href{mailto:vel@latextemplates.com}{Vel} and Johannes Böttcher.

%----------------------------------------------------------------------------------------

\section{What this Template Includes}

\subsection{Folders}

This template comes as a single zip file that expands out to several files and folders. The folder names are mostly self-explanatory:

\keyword{Appendices} -- this is the folder where you put the appendices. Each appendix should go into its own separate \file{.tex} file. An example and template are included in the directory.

\keyword{Chapters} -- this is the folder where you put the thesis chapters. A thesis usually has about six chapters, though there is no hard rule on this. Each chapter should go in its own separate \file{.tex} file and they can be split as:
\begin{itemize}
\item Chapter 1: Introduction to the thesis topic
\item Chapter 2: Background information and theory
\item Chapter 3: (Laboratory) experimental setup
\item Chapter 4: Details of experiment 1
\item Chapter 5: Details of experiment 2
\item Chapter 6: Discussion of the experimental results
\item Chapter 7: Conclusion and future directions
\end{itemize}
This chapter layout is specialised for the experimental sciences, your discipline may be different.

\keyword{Figures} -- this folder contains all figures for the thesis. These are the final images that will go into the thesis document.

\subsection{Files}

Included are also several files, most of them are plain text and you can see their contents in a text editor. After initial compilation, you will see that more auxiliary files are created by \LaTeX{} or BibTeX and which you don't need to delete or worry about:

\keyword{example.bib} -- this is an important file that contains all the bibliographic information and references that you will be citing in the thesis for use with BibTeX. You can write it manually, but there are reference manager programs available that will create and manage it for you. Bibliographies in \LaTeX{} are a large subject and you may need to read about BibTeX before starting with this. Many modern reference managers will allow you to export your references in BibTeX format which greatly eases the amount of work you have to do.

\keyword{MastersDoctoralThesis.cls} -- this is an important file. It is the class file that tells \LaTeX{} how to format the thesis. 

\keyword{main.pdf} -- this is your beautifully typeset thesis (in the PDF file format) created by \LaTeX{}. It is supplied in the PDF with the template and after you compile the template you should get an identical version.

\keyword{main.tex} -- this is an important file. This is the file that you tell \LaTeX{} to compile to produce your thesis as a PDF file. It contains the framework and constructs that tell \LaTeX{} how to layout the thesis. It is heavily commented so you can read exactly what each line of code does and why it is there. After you put your own information into the \emph{THESIS INFORMATION} block -- you have now started your thesis!

Files that are \emph{not} included, but are created by \LaTeX{} as auxiliary files include:

\keyword{main.aux} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

\keyword{main.bbl} -- this is an auxiliary file generated by BibTeX, if it is deleted, BibTeX simply regenerates it when you run the \file{main.aux} file. Whereas the \file{.bib} file contains all the references you have, this \file{.bbl} file contains the references you have actually cited in the thesis and is used to build the bibliography section of the thesis.

\keyword{main.blg} -- this is an auxiliary file generated by BibTeX, if it is deleted BibTeX simply regenerates it when you run the main \file{.aux} file.

\keyword{main.lof} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Figures} section.

\keyword{main.log} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It contains messages from \LaTeX{}, if you receive errors and warnings from \LaTeX{}, they will be in this \file{.log} file.

\keyword{main.lot} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Tables} section.

\keyword{main.out} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

So from this long list, only the files with the \file{.bib}, \file{.cls} and \file{.tex} extensions are the most important ones. The other auxiliary files can be ignored or deleted as \LaTeX{} and BibTeX will regenerate them.

%----------------------------------------------------------------------------------------

\section{Filling in Your Information in the \file{main.tex} File}\label{FillingFile}

You will need to personalise the thesis template and make it your own by filling in your own information. This is done by editing the \file{main.tex} file in a text editor or your favourite LaTeX environment.

Open the file and scroll down to the third large block titled \emph{THESIS INFORMATION} where you can see the entries for \emph{University Name}, \emph{Department Name}, etc \ldots

Fill out the information about yourself, your group and institution. You can also insert web links, if you do, make sure you use the full URL, including the \code{http://} for this. If you don't want these to be linked, simply remove the \verb|\href{url}{name}| and only leave the name.

When you have done this, save the file and recompile \code{main.tex}. All the information you filled in should now be in the PDF, complete with web links. You can now begin your thesis proper!

%----------------------------------------------------------------------------------------

\section{The \code{main.tex} File Explained}

The \file{main.tex} file contains the structure of the thesis. There are plenty of written comments that explain what pages, sections and formatting the \LaTeX{} code is creating. Each major document element is divided into commented blocks with titles in all capitals to make it obvious what the following bit of code is doing. Initially there seems to be a lot of \LaTeX{} code, but this is all formatting, and it has all been taken care of so you don't have to do it.

Begin by checking that your information on the title page is correct. For the thesis declaration, your institution may insist on something different than the text given. If this is the case, just replace what you see with what is required in the \emph{DECLARATION PAGE} block.

Then comes a page which contains a funny quote. You can put your own, or quote your favourite scientist, author, person, and so on. Make sure to put the name of the person who you took the quote from.

Following this is the abstract page which summarises your work in a condensed way and can almost be used as a standalone document to describe what you have done. The text you write will cause the heading to move up so don't worry about running out of space.

Next come the acknowledgements. On this page, write about all the people who you wish to thank (not forgetting parents, partners and your advisor/supervisor).

The contents pages, list of figures and tables are all taken care of for you and do not need to be manually created or edited. The next set of pages are more likely to be optional and can be deleted since they are for a more technical thesis: insert a list of abbreviations you have used in the thesis, then a list of the physical constants and numbers you refer to and finally, a list of mathematical symbols used in any formulae. Making the effort to fill these tables means the reader has a one-stop place to refer to instead of searching the internet and references to try and find out what you meant by certain abbreviations or symbols.

The list of symbols is split into the Roman and Greek alphabets. Whereas the abbreviations and symbols ought to be listed in alphabetical order (and this is \emph{not} done automatically for you) the list of physical constants should be grouped into similar themes.

The next page contains a one line dedication. Who will you dedicate your thesis to?

Finally, there is the block where the chapters are included. Uncomment the lines (delete the \code{\%} character) as you write the chapters. Each chapter should be written in its own file and put into the \emph{Chapters} folder and named \file{Chapter1}, \file{Chapter2}, etc\ldots Similarly for the appendices, uncomment the lines as you need them. Each appendix should go into its own file and placed in the \emph{Appendices} folder.

After the preamble, chapters and appendices finally comes the bibliography. The bibliography style (called \option{authoryear}) is used for the bibliography and is a fully featured style that will even include links to where the referenced paper can be found online. Do not underestimate how grateful your reader will be to find that a reference to a paper is just a click away. Of course, this relies on you putting the URL information into the BibTeX file in the first place.

%----------------------------------------------------------------------------------------

\section{Thesis Features and Conventions}\label{ThesisConventions}

To get the best out of this template, there are a few conventions that you may want to follow.

One of the most important (and most difficult) things to keep track of in such a long document as a thesis is consistency. Using certain conventions and ways of doing things (such as using a Todo list) makes the job easier. Of course, all of these are optional and you can adopt your own method.

\subsection{Printing Format}

This thesis template is designed for double sided printing (i.e. content on the front and back of pages) as most theses are printed and bound this way. Switching to one sided printing is as simple as uncommenting the \option{oneside} option of the \code{documentclass} command at the top of the \file{main.tex} file. You may then wish to adjust the margins to suit specifications from your institution.

The headers for the pages contain the page number on the outer side (so it is easy to flick through to the page you want) and the chapter name on the inner side.

The text is set to 11 point by default with single line spacing, again, you can tune the text size and spacing should you want or need to using the options at the very start of \file{main.tex}. The spacing can be changed similarly by replacing the \option{singlespacing} with \option{onehalfspacing} or \option{doublespacing}.

\subsection{Using US Letter Paper}

The paper size used in the template is A4, which is the standard size in Europe. If you are using this thesis template elsewhere and particularly in the United States, then you may have to change the A4 paper size to the US Letter size. This can be done in the margins settings section in \file{main.tex}.

Due to the differences in the paper size, the resulting margins may be different to what you like or require (as it is common for institutions to dictate certain margin sizes). If this is the case, then the margin sizes can be tweaked by modifying the values in the same block as where you set the paper size. Now your document should be set up for US Letter paper size with suitable margins.

\subsection{References}

The \code{biblatex} package is used to format the bibliography and inserts references such as this one \parencite{Reference1}. The options used in the \file{main.tex} file mean that the in-text citations of references are formatted with the author(s) listed with the date of the publication. Multiple references are separated by semicolons (e.g. \parencite{Reference2, Reference1}) and references with more than three authors only show the first author with \emph{et al.} indicating there are more authors (e.g. \parencite{Reference3}). This is done automatically for you. To see how you use references, have a look at the \file{Chapter1.tex} source file. Many reference managers allow you to simply drag the reference into the document as you type.

Scientific references should come \emph{before} the punctuation mark if there is one (such as a comma or period). The same goes for footnotes\footnote{Such as this footnote, here down at the bottom of the page.}. You can change this but the most important thing is to keep the convention consistent throughout the thesis. Footnotes themselves should be full, descriptive sentences (beginning with a capital letter and ending with a full stop). The APA6 states: \enquote{Footnote numbers should be superscripted, [...], following any punctuation mark except a dash.} The Chicago manual of style states: \enquote{A note number should be placed at the end of a sentence or clause. The number follows any punctuation mark except the dash, which it precedes. It follows a closing parenthesis.}

The bibliography is typeset with references listed in alphabetical order by the first author's last name. This is similar to the APA referencing style. To see how \LaTeX{} typesets the bibliography, have a look at the very end of this document (or just click on the reference number links in in-text citations).

\subsubsection{A Note on bibtex}

The bibtex backend used in the template by default does not correctly handle unicode character encoding (i.e. "international" characters). You may see a warning about this in the compilation log and, if your references contain unicode characters, they may not show up correctly or at all. The solution to this is to use the biber backend instead of the outdated bibtex backend. This is done by finding this in \file{main.tex}: \option{backend=bibtex} and changing it to \option{backend=biber}. You will then need to delete all auxiliary BibTeX files and navigate to the template directory in your terminal (command prompt). Once there, simply type \code{biber main} and biber will compile your bibliography. You can then compile \file{main.tex} as normal and your bibliography will be updated. An alternative is to set up your LaTeX editor to compile with biber instead of bibtex, see \href{http://tex.stackexchange.com/questions/154751/biblatex-with-biber-configuring-my-editor-to-avoid-undefined-citations/}{here} for how to do this for various editors.

\subsection{Tables}

Tables are an important way of displaying your results, below is an example table which was generated with this code:

{\small
\begin{verbatim}
\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}
\end{verbatim}
}

\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}

You can reference tables with \verb|\ref{<label>}| where the label is defined within the table environment. See \file{Chapter1.tex} for an example of the label and citation (e.g. Table~\ref{tab:treatments}).

\subsection{Figures}

There will hopefully be many figures in your thesis (that should be placed in the \emph{Figures} folder). The way to insert figures into your thesis is to use a code template like this:
\begin{verbatim}
\begin{figure}
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}
\end{verbatim}
Also look in the source file. Putting this code into the source file produces the picture of the electron that you can see in the figure below.

\begin{figure}[th]
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}

Sometimes figures don't always appear where you write them in the source. The placement depends on how much space there is on the page for the figure. Sometimes there is not enough room to fit a figure directly where it should go (in relation to the text) and so \LaTeX{} puts it at the top of the next page. Positioning figures is the job of \LaTeX{} and so you should only worry about making them look good!

Figures usually should have captions just in case you need to refer to them (such as in Figure~\ref{fig:Electron}). The \verb|\caption| command contains two parts, the first part, inside the square brackets is the title that will appear in the \emph{List of Figures}, and so should be short. The second part in the curly brackets should contain the longer and more descriptive caption text.

The \verb|\decoRule| command is optional and simply puts an aesthetic horizontal line below the image. If you do this for one image, do it for all of them.

\LaTeX{} is capable of using images in pdf, jpg and png format.

\subsection{Typesetting mathematics}

If your thesis is going to contain heavy mathematical content, be sure that \LaTeX{} will make it look beautiful, even though it won't be able to solve the equations for you.

The \enquote{Not So Short Introduction to \LaTeX} (available on \href{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}{CTAN}) should tell you everything you need to know for most cases of typesetting mathematics. If you need more information, a much more thorough mathematical guide is available from the AMS called, \enquote{A Short Math Guide to \LaTeX} and can be downloaded from:
\url{ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf}

There are many different \LaTeX{} symbols to remember, luckily you can find the most common symbols in \href{http://ctan.org/pkg/comprehensive}{The Comprehensive \LaTeX~Symbol List}.

You can write an equation, which is automatically given an equation number by \LaTeX{} like this:
\begin{verbatim}
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}
\end{verbatim}

This will produce Einstein's famous energy-matter equivalence equation:
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}

All equations you write (which are not in the middle of paragraph text) are automatically given equation numbers by \LaTeX{}. If you don't want a particular equation numbered, use the unnumbered form:
\begin{verbatim}
\[ a^{2}=4 \]
\end{verbatim}

%----------------------------------------------------------------------------------------

\section{Sectioning and Subsectioning}

You should break your thesis up into nice, bite-sized sections and subsections. \LaTeX{} automatically builds a table of Contents by looking at all the \verb|\chapter{}|, \verb|\section{}|  and \verb|\subsection{}| commands you write in the source.

The Table of Contents should only list the sections to three (3) levels. A \verb|chapter{}| is level zero (0). A \verb|\section{}| is level one (1) and so a \verb|\subsection{}| is level two (2). In your thesis it is likely that you will even use a \verb|subsubsection{}|, which is level three (3). The depth to which the Table of Contents is formatted is set within \file{MastersDoctoralThesis.cls}. If you need this changed, you can do it in \file{main.tex}.

%----------------------------------------------------------------------------------------

\section{In Closing}

You have reached the end of this mini-guide. You can now rename or overwrite this pdf file and begin writing your own \file{Chapter1.tex} and the rest of your thesis. The easy work of setting up the structure and framework has been taken care of for you. It's now your job to fill it out!

Good luck and have lots of fun!

\begin{flushright}
Guide written by ---\\
Sunil Patel: \href{http://www.sunilpatel.co.uk}{www.sunilpatel.co.uk}\\
Vel: \href{http://www.LaTeXTemplates.com}{LaTeXTemplates.com}
\end{flushright}


\end{comment}


==> Chapters/Chapter1.tex <==
% Chapter 1

\chapter{Introduction} % Main chapter title
\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\begin{displayquote}
“Intelligence is the ability to reach the same ends by different means”

\raggedleft —William James

\end{displayquote}


% EML makes some misconceptions, but fail to capture biological computation. Genotype is not equal to the Phenotype. A layer of development (competency) exists between the two 
A common misconception in the field of Evolutionary Computation is that the genotype maps directly to the phenotype and that learning is representative of intelligence. While these assumptions have helped solve a range of computational problems, they fail to capture the essence of biological computation. In real biology, no such direct map exists between the genotype and the phenotype, developmental-morphogenesis acts as a layer of control between the two. Importantly, genes do not code for structure and function of an organism; instead, organisms emerge as a result of the complex set of interactions occurring between cellular collectives during morphogenesis. While genomes specify the hardware (in the form of proteins), it is the software (resulting from cellular activity) which is ultimately responsible for an organisms' structure and behaviour.\\

% Cellular competency is problem solving in multiple subspaces
If one were to inspect the activity of cells, a broad picture emerges, where cells coordinate their activity by communicating with each other to solve problems in multiples sub-spaces (anatomical, transcriptional, functional etc..). Further, the capabilities of unicellular organisms hint that cells themselves are not passive materials, but agential substrates capable of complex behavior. The ability of individual cell's to scale their problem solving capability (i.e, their competency/intelligence) to tissues, organs, organ-systems and eventually the whole organism is what gives rise to the functional diversity of an organism, rendering it "intelligent". \\

% Problem-solving influences form-function, therefore it must have an effect on evolution.

Given that developmental-morphogenesis dictates the genome-form-function relationship, it must have significant implications to the evolutionary process itself. This inverse relationship is poorly explored in literature, with a handful of works acknowledging it from the higher-order perspective of learning. The following work is aimed at addressing this issue by treating intelligence as a low-order cellular process termed "competency", and by studying how the scaled-intelligence of cellular-collectives during morphogenesis influences evolutionary dynamics. 


\section{Research Motivation}

Understanding the effects of cellular competency/intelligence on evolution can augment our current knowledge on several fronts: 

\begin{itemize} 

    \item It can encourage development of a new class of evolutionary algorithms, where genomes act as subjects of evolution, separated from the functional outcome by means of a developmental process. Such a framework could help us \textit{grow} collective-intelligences capable of exhibiting the robustness and the plasticity of real world biological organisms.

    \item It can shed light on confounding morphological phenomenon in Biology, such as that of the highly regenerative planarian: due to reproduction by fissioning and regeneration, planaria retain mutations made in its parent body and pass them on to their offspring. As a result planarian have a messy genome, with different chromosomes in each cell. Despite this, they have the most reliable anatomy: every fragment of a planarian reliably regenerates to a perfect worm each time. How does evolution ensure reliable anatomy given such a chaotic genome? 
    
    \item  It is currently impossible to guess the anatomy of an organism by examining its genome. If one were to combine the genomes of two known organisms in equal proportion there is no way to predict the resulting anatomy: would it have features similar to either of its parents? What would its functional capability be? We lack sufficient knowledge of the developmental process to answer such questions. A key aspect here is the origin of the developmental process itself: how does evolution optimize the manner of self-organization carried out by the developmental process? 
    
\end{itemize}

\section{Research Question}
The main question we address here is:

\begin{itemize}
    \item How do diverse levels of competency in the cellular collective during morphogenesis impact the rate and course of the evolutionary process? 
\end{itemize}

\section{Hypothesis}

We approach our research question with the assumption that competency is beneficial to developmental-morphogenesis, with the capability to significantly alter the evolutionary dynamics of a population. Given this assumption, we make the following hypotheses:

\begin{itemize}
\item[1.] Populations with a greater degree of competency reach morphological goals faster than those with a lesser degree of competency.

\item[2.] Given a choice between several degrees of competency, evolution prefers to select for the highest competency. 

\item[3.] In a mixed population composed of both competent and non-competent individuals, evolution prefers to select for competent individuals.

\item[4.] Competency helps evolutionary algorithms escape local minima.

\end{itemize}

\section{Research Objectives}

\begin{itemize}
    \item Develop a modular software framework for the manipulation of artificial embryos.

    \item Introduce the developmental process as a novel step in the iterative sequence of a standard genetic algorithm.

    \item Develop a global fitness function capable of assessing the morphological state of an artificial embryo. 

    \item Examine the role of hyper-parameters on the dynamics of evolution.

    \item Discuss limitations of the proposed framework. 
\end{itemize}


\section{Main Contributions}

We develop a software framework to simulate the morphogenesis of virtual-embryos in-silico. A virtual embryo is a 1-dimensional array of integers (analogous to cells), with the integer sequence from left-to-right representing the morphology of the embryo.

We evolve populations of virtual-embryos by means of a modified genetic algorithm involving the iterative steps of: Development, Selection, Mutation, and Crossover. The developmental step is defined so as to permit communication between individual cells leading to their reorganization within a \textit{local} neighborhood. Post Development, a global fitness function assesses the degree of monotonic order within cells of the virtual embryo. Results from our simulations reveal the extent to which competency impacts evolution, and provides explanations for the confounding nature of planaria. We discuss possible extensions to our methodology, highlighting the applicability of competency to the fields of artifical life and evolutionary robotics.

\section{Outline}







% Questions addressed: Refer notes + paper: Clearly state your research questions, clearly state your research objectives and hypothesis. State clearly the contribution of your dissertation to the universal body of knowledge. 


==> Chapters/Chapter2.tex <==
% Chapter Template

\chapter{Related work} % Main chapter title

\label{Chapter2} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}


\section{Background}

\subsection{Evolutionary Computation}

Evolutionary computation is a sub-field in Artificial intelligence which adopts techniques from biological evolution to solve computational problems. Of particular interest to our discussion here concerns works which try to capture biological intelligence by simulating Darwinian evolution in general purpose computers. 

Genetic algorithms are a class of evolutionary algorithms which are particularly employed to this end. A standard genetic algorithm evolves a population of "individuals", whose functional-outcome (i.e, the phenotype) is determined by a genotype which specifies the structure of the function producing the outcome. Evolution occurs through the iterative application of three major steps: 

\begin{itemize}
    \item[1.] Selection: During which functional-outcomes (phenotypes) of each individual (as determined by its genotype) is assessed by a fitness function and the genotypes of those individuals which produce the best functional-outcomes are chosen to move onto the next iteration/generation, with the inferior genotypes being excluded from the population. 

    \item[2.] Mutation: The selected genotypes are stochastially modified to a random value, 

    \item[3.] Cross-over: To repopulate the selected population back to its original strength, a reproductive process ensures, during which the best individuals "mate" with each other to give rise to new genotypes which are an arbitrary combination of its parents. 
    
\end{itemize}

The genetic algorithm serves as a rough approximation of Darwinian evolution as observed in nature. However, a major aspect of Darwinian Evolution ignored in genetic algorithms is the fact that biological phenotypes are \textit{emergent} in nature. Crucially, the genotype cannot be allowed to explicitly map to the phenotype. If it were, the behaviour and function of biological organisms would be pre-determined and fixed. 

Phenotypes are functional \textit{outcomes} of development, during which the components encoded by the genotype interact with one another, and self-organize into a morphological structure capable of plastically processing information from its external environment.

This fact is not completely ignored in literature. Several works do acknowledge the developmental process as a layer between the genotype and the phenotype, however, they all do so by substituting the developmental process with learning. Learning is clearly a process of intelligence, but it is an emergent outcome of development, manifesting at the level of the organism. There must be a low-level phenomenon giving rise to such an ability. 

Seeking the source of emergent outcomes, leads us to ask the question: where does "intelligence" actually emerge i.e, at what level of a biological organism do fundamental aspects of physics, chemistry, and biology transition into an autonomous, problem-solving entity? A step towards answering this question comes from first defining intelligence. Several works have tried to provide a formal definition of the matter, the one we use here is a version defined by Francois Chollet:  "Intelligence is information processing capability leading to efficient, generalizable problem solving in multiple domains". Importantly, intelligence is not a binary quality, but exists on a continuum of degrees.

Given this definition, we can move down the complexity hierarchy of a biological organism to investigate where the least possible degree of intelligence manifests. The answer to this question as it turns out is a cell. 

The following subsections describe how intelligence manifests at the level of a cell, and the role developmental-morphogenesis plays in scaling intelligence from the cellular level to that of an organism. 

\subsection{The Cell: a vessel of information processing hardware}
% What are cells? what are organelles? 
% Prokaryotes > Eukaryotes > Cells > 

Biological organisms, regardless of being prokaryotic or eukaryotic, unicellular or multicellular, begin life as a single cell. In multicellular organisms, cells divide to give rise to functional structures, whereas single-celled organisms are autonomous entities themselves. Single celled organisms despite their simplicity, are complex functional units. For instance, Bacteria -- the most primitive prokaryotic organisms -- are capable of metabolising nutrients, attaching themselves to surfaces, swimming through liquids, escaping predators, and reproducing. They are even capable of aggregating themselves and behaving as a multi-cellular collective. Amoeba, a class of eukaryotic organisms can morphs their shape to navigate complex environments. Physarum polycephalum -- yet another, eukaryotic single celled organism -- is capable of detecting objects in its surroundings, and can even solve the shortest path problem. 

These abilities require cells to manipulate information from their environment in goal-directed ways. Such complex information processing is possible because of two crucial moieties within the cell: 1. A structural communication network facilitating signal transport from one region of the cell to another, and 2. Detection mechanisms which help the cell detect information flowing in such a network.

Proteins are a class of macro-molecules responsible for both. In addition to their role in communication, they help catalyze reactions within the cytoplasm and cell-organelles, essentially transducing signals from one form to another. 

Structurally, proteins are formed when amino-acids (bio-molecules with distinct chemical properties) chain together in specific sequences as directed by the cell's genome. The manner in which amino-acid are linked together matters because it results in conformational changes of the chain, causing it to twist and fold at different locations, giving rise to a 3-d structure which determines the protein's function: enabling it to act as an enzyme, as a structural or transport material, or as a bio-molecular detector. 

Proteins, together with cell organelles, and the cell-membrane form a complex information processing unit. 

    % * Define information

% The genotype: Definition, how the DNA carries it, and what information it carries.

\subsubsection{The Genotype: a recipe for cellular hardware}

Proteins are manufactured within a cell based on instructions encoded in the cell's genotype. The genotype refers to the set of all genes contained in an organism. In most biological organisms, the DNA is the structure which carries this information within the Nucleus of a cell. 

DNA -- Deoxyribonucleic-acid -- is an organic polymer composed of two polynucleotide chains. Each strand of DNA is made up of monomeric nuleotides, named based on one of four nitrogen bases it carries (adenine, guanine, cytosine, or thymine). The nitrogenous bases of the nucleotides in one strand bond to the nitrogen bases of nucleotides in the other strand to form the double helix distinctive of DNA. 

The sequence of nucleotides on any \textit{single} strand of DNA encodes genetic information in the form of short nucleotide sub-sequences (genes). Genes  act as instructions to weave-together amino-acids thereby forming a protein. A single strand of DNA carries multiple genes (usually in the order of thousands) so as to be capable of manufacturing a variety of proteins.

% The phenotype: Define it, provide examples

\subsubsection{The Phenotype: observable outcomes of genes}

The phenotype is generally taken to indicate \textit{any} product, direct or indirect, emerging out of the genotype: the 3-d stucture of synthesized proteins, the morphology of the organism, its behavior, and even products of an organism's behavior (such as societal culture). 

\subsubsection{The layer between the genotype and the phenotype}

Despite its broad definition, the phenotype fails to address \textit{how} functional-products emerge from the genotype. This question is fairly complex because it has several layers to it: If one were to look immediately post DNA-translation, it would be obvious to claim that the 3-D structure of a protein emerges because individual amino-acids in the amino-acid-chain repel/attact each other to fold specifically. However, the further in complexity we progress, a logical answer escapes observed phenomenon. One common example which is relevant here is that of morphology: How does the genotype (which encodes for proteins in individual cells) determine the global shape and structure of an organism? Given that there exists a close relationship between form and function answering this question becomes essential to understand the genotype-phenotype relationship. 

In animals, development begins when the male gamete (sperm) fuses with a female gamete (ova) to give rise to the single-celled zygote. Development post this stage involves a complex sequence of steps where cell-fates are determined through differentiation (Patterning), organized in space-time (Morphogenesis), and restructured (Tissue growth) to give rise to a mature embryo. Each of these processes are far from independent, occurring simultaneously in a manner integrated across space as well as time, their coordination being the main reason for their success. Such coordination is possible because of communication networks established by cells, facilitating transmission of bioelectric and biochemical signals across space to ensure reliable development. 

Biochemical signalling is brought about when an endogenous signalling molecule is detected by a cell and transported into its cytoplasm to initiate a sequence of chemical reactions resulting in a functional product. Such a signalling mechanism is particularly effective for short range communication, because of the dwindling concentration of the signalling molecule. 

Bioelectric signalling on the other hand is brought about by electric currents circulating between cells. Fundamentally, bioelectricity arises because of a difference in ion concentration between the interior and exterior of a cell, caused by the isolation of the plasma membrane acting as a capacitor. Several structural proteins (ion-channels, ion-pumps, exchangers, and transporters) embedded in the bi-lipid plasma membrane transport and diffuse ions between the cell and its external environment giving rise to a resting membrane potential ($V_{mem}$). 

Every embryonic cell possess a $V_{mem}$ which can be broadcasted across large distances through gap junctions prevalent between neighboring cells. Essentially, each cell can act like a battery, connecting itself with other cells to generate different voltages and electric fields. Also, since gap-junctions and ion-channels are themselves voltage sensitive, cell groups can self-organize to from complex electric circuits with rich feedback capabilities. These circuits give rise to intricate, dynamic voltage gradient patterns which demarcate anatomical features and act like blue-prints for gene-expression and morphogenesis during embryonic-development. Bioelectricity even has the capacity to serve as a secondary messenger: capable of being transduced into bio-chemical signals and influencing transcription networks. 

Regardless of the manner of signalling, the communication networks established by cellular collectives are \textit{emergent}, arising out of self-organization between local cells-groups. The genotype does not encode information about the  manner in which communication networks are to be established during development. Concrete evidence exists to this end.

\begin{itemize}
    \item[1.] Bioelectric patterns \textit{during} development can be tampered with to give rise to radically different morphological outcomes without any change to the genome itself: 

    \begin{itemize}
        \item experimental modifications of endogenous bioelectric patterns in-vivo during development of xenopus laevis embryos (frog embryos) have enabled growth of functional eyes on tails and in gut tissue of the resulting tadpoles. 
     
        \item editing bioelectric gradients during planarian development has led to the growth of two-headed planarian, with reversal of the bioelectric edit resetting normal development. 
    
        \item tampering with bioelectric networks has led to conversion of flatworm head shapes to different species-specific head anatomies and has even induced regeneration of appendages in tadpoles which were otherwise non-regenerative.

    \end{itemize}

\end{itemize}    

    \noindent In each of these examples, it must be emphasized that, the phenotypes which emerged as a consequence of bioelectric edits were novel, never before seen in the organism's evolutionary history.
    
\begin{itemize}
    \item [2.] Lack of correspondence between the genotype and morphological-complexity: Over the past sixty years, the genomes of a wide variety of plants, animals, and fungi have been mapped, yet there exists no relationship between the size of the genome and the complexity of an organism, especially amongst eukaryotes. For instance, Protopterus aethiopicus, the marbled lungfish has 40 times the amount of DNA per cell compared to humans. 
    
    \item[3.] Behaviour -- the unique manner in which an organism interacts with its environment -- is itself a phenotype, and is significantly shaped by the external environment. Given the amenable nature of behaviour in living organisms, it is unlikely for the genome to have played a restrictive role in its manifestation. 
    
\end{itemize}

These observations reveal the breadth of disparity between the genotype and the phenotype, further clarifying that the genome's involvement is solely in constructing cellular hardware by manufacturing proteins, with the morphology and function of an organism emerging as a result of development during which cell groups communicate with each other to signal their collective states to achieve anatomical goals. 

% mention environmental effects

% The developmental process: Mention that a lot of things occur between the expression of proteins and its manifestation as an observable trait (the intermediate layer b/w genotype and phenotype). Take it from the cell-first, how protein expression is dictated by surrounding cells, talk about how bioelectricity is a key communication entity for a cell to understand what to do when (cite examples about how eyes can be grown on tails and broke a pre-conceived notion that eyes have to grow closer to the head). Talk about how bioelectricity influences regulation within the cell (gene-regulation). Highlight that the developmental process can be tampered with by hacking into a cell's bioelectic signals. 

    % * mention implications of the genotype neq phenotype: Cannot guess the anatomy by examining an genome

\subsection{Cells are not passive, but agential materials}

Importantly, the cells which make up multi-cellular organisms are themselves independent, having evolved from unicellular organisms with extensive capabilities for sensing and responding in their environment. These cells do not lose their independence when part of a collective: isolating skin cells of the Xenopus Laevis embryo from its collective, causes it to  exhibit unassisted movement. It is even possible to craft a new organism from embryonic cells of the xenous laevis embryo capable of exhibiting novel behaviors. 

It seems that cells tend to serve their own goals when left alone, executing a wide range of functions to scavenge, move, and reproduce. However, as part of a collective, their functionality is rewired to solve tasks which ensure survival of the whole.

Crucially, individual cells maintain functional homeostasis by solving problems in multiple sub-spaces (transcriptional, anatomical, functional, etc..). Problem solving in each of these domains is interrelated, often occurring simultaneously. We refer to this multi-dimensional problem solving capability of individual cells as competency and believe that competency is representative of intelligence.

Competency itself can occur at multiple-scales: at the level of cells, at the level of tissues, and at the level of organs. The manner in which competency scales from an individual cells to cellular-collectives is determined during morphogenesis. Given that this rapid, built-in, capacity for anatomical homeostasis determines the form of an organism and consequently its function, it must have implications to the evolutionary process which crafts its behaviour.

% Cells as agential materials: Talk about how bioelectricity is what makes cells cooperate with the whole, if left alone they do their own thing, indicating that cells are active agential elements themselves. Talk about multiple examples where this is true (refer to your notes). Mention competency for the first time and cite the planaria to claim why random mutations need not be disastrous (because competency can make up for the chaos). Define competency and cite some examples (refer notes). Claim that competency plays a major role in anatomical homeostasis and must have important implications for the evolutionary process itself.


\section{Related work}


% Refer to history from: peter ternet, 1996: Lamarck's view, but not true, so how is progress actually made? (c.morgan), Darwin's NS theory. An important aspect is the inheritence of those traits which are not explicitly encoded by the genotype: the canalization of accquired tratis through the baldwin effect (baldwin + c.lloyd morgan): experimental evidence by waddington that canalization occur over a long period of time. Introduce evolutionary computation. Simulated evidence to show how adaptation can alter evolution, essentially making it efficient (hinton  + everyone else in the mayley 1996 paper), learning was treated as the key adaptable trait and its effect on evolution was studied (larry Bull, 1999 paper; stefano nolfi + the ones mentioned in mayley 1996): showing how learning can complement evolution. A slew of work is cited in Peter turney, 1996: Harvey's experiments of learning one evolution, the motivation system in RL, Baldwin effect in visual concept recognition, baldwin effect as a possible dynamic bias knob for ML. How competency is different from learning (check your paper). 

% Mention the nature of the genetic algorithm used as a version by Holland. Mention the role of hyperparameters (studied by Belew, 1990 for hinton's paper).


% behavior which boosts fitness can eventually get assimilated in the genotype (baldwin)

% Waddingtion exhibits a similar phenomenon where environment induced phenotypes are canalized into the genome of in-vivo flies. 

% Hinton's seminal paper showing how lifetime-learning/behavior based on the baldwin effect can influence evolutionary dynamics.

% The computer science community goes on to assess the imnpact of intelligence on evolution exclusively from the perspective of NN development.

% 
\subsubsection{Baldwin Effect: the effect of intelligence on evolution}

Many organisms can modify their behavior in the light of experience, improving their fitness via information that was not provided by the genome. Baldwin was the first to record such an observation as early as 1896, noting that lifetime behaviors beneficial to an individual are assimilated in the genome over evolutionary timescales (known as the baldwin effect). A decade later, waddington, independently showed that advantageous phenotypic traits acquired as a result of the environment, could be canalized into the genome over the course of evolution. These two  observations gave way to the general consensus that phenotypic traits beneficial to an individual during its lifetime, can get genetically hardwired into the genome over evolutionary timescales thereby significantly altering evolutionary dynamics.\\

Artificial intelligence during the late 20th century was in its exploratory phase. Computer scientists were actively trying to improve the capabilities of neural networks, with the goal of trying to capture human-intelligence. A constant source of inspiration during this period came from the field of evolutionary biology, which sought to understand the functional capabilities of evolution through the lens of natural selection. \\

Hinton and Nowak, were the first computer scientists to assess the impact of phenotypic traits on evolutionary dynamics in-silico. They compared the evolution of two populations: one with a standard genetic algorithm, and the other with a learning process accompanying the genetic algorithm. Results from their model indicated that local search methods such as individual-level learning could significantly change the search space; essentially guiding the global search (carried out by evolutionary algorithms) towards an optimal solution. \\

Spurred by these results, the computer science community began investigating the baldwin effect in depth: Multi layer perceptrons evolved with a genetic algorithm and gradient based learning were shown to evolve faster. Studies confirmed that evolution and learning influenced each other in bidirectional ways. The impact of the learning algorithm, as well as the learning rate on evolution was recorded. Several works even studied the impact of learning in dynamic environments. Results from all of these experiments confirmed what was originally hypothesized by hinton et al: learning could guide evolutionary search towards an optimum solution better than its non-learning counterparts.\\ 

During the same period, a number of works probed the conditions for the origin of the baldwin effect. It was shown that genetic assimilation occurred only when there were costs associated with the phenotypic adaptive process. For instance: If learning helped an individual survive, it came with the cost of acquiring knowledge. Therefore, for the benefit of future populations, evolution would be under selective pressure to hardwire traits which facilitate learning into the genome. Next, a high correlation between the task space (over which adaptive processes operate) and the evolutionary search space was shown to be a prerequisite for the baldwin effect. The rate and magnitude of the adaptive process, and the environmental complexity was shown to matter as well. Several studied even found the manner of reproduction (sexual or asexual) employed in the genetic algorithm to have an effect, with sexual reproduction ensuring genetic assimilation to a greater degree.\\ 

Evolutionary algorithms are fundamentally function optimization algorithms, it would be interesting to have an understanding of how the baldwin effect intervenes with the optimization process. Whitley et al carried out such an assessment. The authors compared lamarckian and baldwinian evolution by optimizing multiple pre-defined functions and showed that a genetic algorithm combined with local search could converge to the global optimum, whereas methods with just the genetic algorithm or larmarckian evolution converged only to a local optimum. 

%Detractors of the Baldwin effect are few, a notable mention from the biological community is that by T. Price etal, who study the role of phenotypic plasticity on evolution in bird populations. Based on their observations, the authors conclude that other factors indirectly related to phenotypic traits could be influencing evolution rather than the phenotypic trait itself. 

\subsubsection{Biological intelligence lies at the cellular level}

The baldwin effect is proof that even though evolution is typically used to evolve adaptive processes, the adaptive process itself can significantly influence evolution. Most of the works presented so far consider gradient-based-learning to be the main adaptive process. The rationale behind this choice being that learning can be taken to represent a wide range of phenomenon during the lifetime of the individual, including its development, growth, intelligence, and any other adaptive trait. Further, the populations being evolved in most of these works are neural networks, where learning is a default sub-routine.\\
   
Neural networks and biological organisms have very little in common. Indeed, neural network based models do not concern themselves with trying to replicate biological organisms, because they can efficiently deploy gradient based learning to exhibit similar task solving capability (i.e, intelligence). We however, believe that efforts to capture intelligence should seek to emulate the self-organization process in biology because every observable adaptive trait is an outcome of morphological development. In spirit of this observation, we acknowledge intelligence as a process which exists at the cellular level; where cells behave as autonomous agents, driven towards their own goals by solving problems in multiple domains (transcriptional, anatomical, behavioural etc..). During developmental-morphogenesis, individual cells communicate with each other to scale their competencies/intelligences to that of the collective whole. \\

The intelligence or the competency of cells is fundamentally different from learning. First, the ability of cells and tissues to attain and maintain setpoints in morphological spaces is independent of learning at the level of the individual. Second, learning at the level of the organism needs a mechanism (e.g., nervous system architecture) that must itself be painstakingly evolved—evolution must discover, maintain, and pay the costs of new capabilities such as brains and exploratory behaviors. In contrast, cellular competencies come “by default” because organisms consist of cellular components that already have many capabilities evolved during their ancestral lifetime as independent organisms. Thus, it is important to begin to study how cellular competencies affect evolution, to complement approaches focused on learning and the material properties of morphological computation. \\

We develop a simplified model to study the role of competency on evolution. Our model seeks to represent a bare minimum of the morphogenetic process as observed in real biology. Our goal is to observe the role of morphogenesis on evolution by applying a genetic algorithm in-silico. In our framework, we treat each individual as a collection of cells. Cells in our model do not have the capacity to divide, so an individual retains a constant number of cells from birth unto death. Each cellular collective at birth is termed an "embryo". Post birth, cells of an embryo undergo morphogenetic development during which cells communicate with each other to rearrange themselves within their respective local areas. Therefore, by design, each cell has an inbuilt goal to rearrange itself by communicating with its local environment. We believe this captures two main components which real cells themselves exhibit: 1. agential behaviour towards a self-serving goal and 2. the ability to communicate with an external environment to coordinate goals.\\ 

A genetic algorithm is tasked with selecting embryos which best organize themselves in the desired pattern. Two main search processes exist in our framework: first, a global search process carried out by the fitness function, and, second, a local search process as a result of the goals sought by individual cells. No external environment is considered. 

We describe our framework next. But before we do so, it must be noted here that our methodology borrows heavily from previously published work of which I was a significant contributor of. 

==> Chapters/Chapter3.tex <==
% Chapter Template

\chapter{Methods} % Main chapter title

\label{Chapter3} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

We simulate the evolution of artificial 1-dimensional embryos in silico. The following sections describe the structure of each embryo, our paradigm for modeling developmental morphogenesis towards a target adult anatomy, and the process of selection employed to study their dynamics over time.

\subsection{Creating Populations for Evolution}
A population consists of a number of embryos. Each embryo is represented as a one-dimensional array of fixed size (matching the cell count in the 1-dimensional embryo). Each cell of this array is initialized with a different integer value representing the positional value gene for the corresponding cell of the embryonic axis (see Appendix A1). In this minimal model, there is no further chromosomal structure or transcriptional change, and we simply refer to the structural genes as directly specifying the positional preference of a given cell. Each embryo undergoes a developmental cycle (described below) to become a mature “individual”. We model evolution in three kinds of populations: a “hardwired” population consisting of only hardwired embryos, a “competent” population of only competent embryos, and a “mixed” population which contains both kinds of embryos, in varying proportions. Our mixed populations have 200 embryos, the rest have 100.

\subsection{Hardwired and Competent Embryos}
We define two types of embryos, a “hardwired embryo” and a “competent embryo” (Figure 1A, B). The difference between them lies in the way they develop during the evolutionary cycle. A competent embryo consists of cells capable of sensing neighboring cells and adapting morphology by moving around \textit{locally} prior to the adult stage in which fitness is evaluated. “Competency” is the capability of these embryos to carry out such reorganization, and they carry a gene (competency gene) that dictates the frequency at which they can do so (fixed, in some experiments, but free to evolve in others). Our competent embryos leverage sensing and motility to reorganize their cells during ‘development’ in a way that boosts fitness (see below and Appendix A1). We vary the degree to which they can reorganize (competency level). A hardwired embryo lacks this capability; its structure from birth to maturity is constant.

\begin{figure}[!h]
\includegraphics[width=13cm]{Figures/Figure 1 - Competency.png}
\centering
\caption{}
\label{Fig: main-methods}
\centering
\end{figure} 

\subsection{Developmental Cycle}
Soon after initialization, embryos undergo a developmental cycle. During this process, competent (but not hardwired) embryos undergo a restricted bubble-sort procedure (see Appendix A1) to rearrange their cells in a way that boosts fitness (i.e., to increase ascending order of its array of integers). At the end of the developmental cycle, embryos are considered “individuals”.

\subsection{Fitness of Embryos and Individuals}
We define fitness as the degree to which an embryo’s array of integers is in ascending order. Individuals with cells arranged in ascending order by value are attributed a fitness of 1.0 (maximum), those whose cells are randomly ordered are attributed a fitness of 0.5. We calculate the fitness (the degree of order) of an array by counting the number of non-inversions present (see Appendix A1). At the beginning of each evolutionary cycle, all embryos are considered “just born”; their morphological structure determined by their parents from the previous generation. Therefore, we call their fitness at the start of each cycle the \textit{genotypic fitness}. At the end of the developmental cycle, the fitness of each resulting individual is calculated again, which we call the \textit{phenotypic fitness}. For hardwired individuals, phenotypic and genotypic fitnesses are always identical. For competent individuals, however, phenotypic fitness reflects the reorganization that occurs based on their competency level.

\subsection{Competency Level}
At the start of each developmental cycle, a competent embryo is assigned an integer representing its competency level. This integer determines how many successive bubble-sort swaps will take place during its developmental cycle. Usually, competency levels are much lower than the total number of bubble-sort swaps required by an embryo to attain maximum fitness, for this reason it is called “restricted” bubble-sort.

\subsection{Competency and intelligence}

Based on our definition of intelligence in Chapter 2, we consider competency to be analogous to intelligence throughout our framework. Both terms are implied to mean the ability of the attributed entity to solve problems in multiple-dimensions, efficiently, with an ingrained agential tendency to solve its own goals. Biological cells are typical examples of such task solving ability. In our framework, cells of a competent embryo solve problems in a single dimension (morphological), but are agential: they have a tendency to reorganize themselves by swapping their positions with  neighbors, and have the capacity to communicate locally. 


\subsection{Genetic Algorithm}
To evolve populations (hardwired or competent), we employ a modified version of the genetic algorithm with the following steps (Figure 1C):
\begin{itemize}
    \item Development: Post initialization, embryos undergo development. A competent embryo reorganises its cells based on the competency value, whereas a hardwired embryo does not. 

    \item Selection: The fittest 10\% of individuals in a population are selected to move on to the next generation. Selection in a population is based on its individuals’ phenotypic fitness (darwinian selection). 

    \item Cross-Over: In order to repopulate a population back to its original strength, we carry out a process of reproduction called cross-over. It occurs as follows: Two individuals are involved, each of these are split at a random location along their length. One half of Individual 1 is swapped with the same half of Individual 2 to give rise to two children. Figure 1 contains an illustration of this process.

    \item Mutation: The repopulated population is subjected to random point mutations. We set the probability of an individual receiving a point mutation to be 0.6.
\end{itemize}


Next, we describe results from our experiments. Once again, we would like to make it clear that a significant part of the results section borrows from previously published work of which I was a major contributor of.

==> Chapters/Chapter4.tex <==
% Chapter Template

\chapter{Results} % Main chapter title

\label{Chapter4} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

We built a virtual embryogeny model in which fitness was defined by the degree of monotonicity of a 1D array of numbers, simulating a minimal organism with a single axis of positional information (Figure 1). The initial sequence of numbers for each embryo was assigned randomly. Since these sequences decided the embryo’s structure (cell order), they are referred to as its structural genes. As described in chapter \ref{Chapter3}, the structural gene sequence of hardwired embryos is fixed: their genome directly encodes for their phenotype. For competent embryos, we implemented different degrees of competency during a developmental period in which cells were allowed some degree of movement relative to their neighbors, allowing them to reorganize to improve monotonicity prior to evaluation of phenotypic fitness. This enabled phenotypic fitness for competent individuals to diverge from raw genotypic fitness, with the extent of divergence depending on how much cell movement was permitted. This corresponds to different degrees of capacity for cells in-vivo to optimize homeostatically preferred local conditions with respect to informational signals such as positional cues and polling of neighboring cell states. An evolutionary cycle was implemented around these developmental events.\\ 

In the initial experiments, the competency gene was fixed to a pre-determined value across the evolutionary run, enabling study of the evolutionary dynamics over time as a function of different degrees of cellular competency.

\subsection{Developmental Competency Accelerates Evolutionary  Search}
We first compared, over 250 generations, the time-course of evolutionary search towards a fully ordered axis in hardwired vs. competent individuals. After 100 generations, the hardwired population had the least fitness compared to populations with varying degrees of competency (Figure 2 and Table 1). Table 1 provides a summary of the generation number at which each population crossed different fitness thresholds. We compared fitness of the best individual in competent and hardwired populations at generations 2, 10, and 20 (because these points exhibited the greatest sample variances.) At each of these, the difference in fitness between hardwired and competent populations was significant (p-values  $\ll 1 \times 10^{-3}$ for all points, Student’s t-test; for details see Appendix A2.1.1).\\

Figure 2 also shows that the 95\% confidence interval bands over 100 repeat runs decreased with increasing competency level, suggesting that more competent architectures are also more consistent in performance over time. Note that hardwired individuals gradually improved to reach peak fitness, taking well over 200 generations to do so, whereas the most competent individuals (with a competency level of 400) did so in under 6 generations. These data demonstrate the role competency plays in non-linearly improving the rate of fitness of a population and support a clear conclusion: the higher the competency, the better the performance.\\

Based on the impact of competency, one could hypothesize that progressively increasing competency would lead to a progressive decrease in selective pressure for good structural genes to appear. An embryo with high competency would have no selective pressure to improve its structural genes beyond a certain level because it can rely on its competency to re-order its cells to reach peak fitness. This is in fact what we observed (Figure 3). We compared the genotypic fitnesses of the best individual in three populations with different levels of competency (20, 100, and 400) to that of a hardwired population. In all three competent populations, genotypic fitness rose with that of the hardwired population for a few generations, after which it plateaued, indicating that at this point, the structural genes were good enough for competency to achieve a phenotypic fitness that insured selection. Further, with increased competency, the 95\% confidence interval bands for genotypic fitness grew wider. Thus, as hypothesized, increasing competency in our simulation enabled excellent performance but reduced selective pressure on the embryo’s structural genes.


\subsection{Competent Individuals Take over Mixed Populations}
Given these tradeoffs, we next asked how mixed populations (200 embryos per population) of competent and hardwired embryos would evolve (Figure 4). We varied both the level of competency and the percentage of competent embryos in the hybrid population at the start of the simulation. To probe the levels of competency required for embryos to dominate the population over the evolutionary simulation, competent embryos were always initialized as a minority of the starting population. Relationships between competency, initial population proportion, and dominance were observed over several runs.\\

When competent embryos constituted just 2.5\% of the initial population, they failed to dominate even at the highest level of competency tested: embryos with a competency level of 95 merely reached equal percentages with hardwired embryos. As their initial proportion in the population increased, competent embryos required progressively less competency to dominate over their hardwired competitors. At 10\%, embryos with a competency level of 75 could dominate; at 20\%, the competency level required for domination decreased to 40; and at 30\%, competent embryos dominated with a competency as low as 10 (Figure 4). In all starting conditions that resulted in dominance of competent embryos, it occurred rapidly, in just two or at most three generations (Table 2).

\subsection{Evolution Prefers a High, Constant Level of Competency}

To determine how competency might spontaneously evolve over generations, we introduced competency as an evolvable trait by letting each embryo’s competency level be determined by a single ‘competency gene’ with value in the range $[1, 500]$. During initialization, the competency genes of all embryos were set randomly to low values in the range $[1, 15]$. Then, during evolution cycles, we allowed each competency gene to be mutated, potentially taking values across the range of $[1, 500]$, and tracked the competency gene values of the best individual over 1000 generations (Figure 5). The prevalence of the competency allele rapidly rose, meandering and exploring values up to 485 during evolution (shaded area in Figure 5A) before plateauing at ~470. We provide a possible explanation for this outcome in the Discussion section.\\

To understand how allowing the competency gene to evolve over 1000 generations affects genotypic fitness, we looked at the phenotypic and genotypic values for the fittest individual in each generation (Figure 5B). Values for the fittest individual quickly settled at consistent configurations in which the phenotypic and genotypic fitnesses diverged considerably. This is a fascinating outcome because it suggests that a certain level of competency reduces the pressure for improvements in an embryo’s structural genes. Once selection can no longer distinguish whether fitness is achieved by a set of good structural genes or by a high competency level that compensates for a poor set of structural genes, it can only improve the population by increasing competency, not by selecting better genetics.\\

To quantify this effect and determine how well selection, which ‘sees’ phenotypic fitness only, selects for genotypes when competency is allowed to evolve, we plotted the degree of correlation between genotypic and phenotypic fitness for all individuals in these populations (Figure 5C). Correlation dropped to 0 within about 20 generations as individuals who succeeded because of their developmental competencies rapidly dominated the population. We conclude that allowing competency to evolve disrupts the ability to select for the best structural genes. We further validated this by examining the frequency, over 1000 cycles of evolution, with which positional changes to a single ‘cell’ resulted from tweaks to the competency gene vs. from tweaks to one of the structural genes. Figure 6 shows that the frequency of changes to the competency gene was much higher than the average of all fifty structural genes across 1000 generations in our simulation.


\subsection{Costs to Competency Ensures Genetic Assimilation: The Baldwin Effect}

The Baldwin Effect, as previously discussed, is the now broadly accepted fact in which individual organisms can achieve greater reproductive success based on behavioral adaptations, and that these adaptations can eventually become hardwired into the genome in subsequent evolutionary cycles. \\

Our initial simulations of the evolutionary impact of cellular competency did not exhibit the Baldwin Effect. This could have been due to the fact that our minimal model did not simulate any cost associated with increasing cellular competency, and thus there was no selective pressure towards genomic changes. Although the actual energetic (or other) costs of cellular competencies are not known for any living model system, it is possible that the cellular computations required for axial patterning require additional resources over and above developmental events (competent or not) that are essential for any embryo. Thus, we next studied the effects of introducing a competency cost by penalizing the fitness of embryos in our model by a factor of their competency-value. Using penalty factors in the range of $[1 \times 10^{-7}, 0.5]$, we did see a Baldwin effect: the rate of rise of genotypic fitness corresponded positively with the increase in penalty factors. For penalty factors over 0.5, the genotypic fitness rose well above the phenotypic fitness, leading to disappearance of the Baldwin effect. \\


The results of simulation using a penalty factor of $1 \times 10^{-4}$ over 3000 generations are shown in Figure 7. As described above for simulations with no competency cost, phenotypic fitness reached its maximum in under 20 generations. However, unlike the previous experiment, the fitness of the structural genes did not plateau after a brief increase, but continued to improve over the course of evolution (Figure 7A). Further, as the genotypic fitness rose, selection preferred progressively lower competency values (Figure 7B). Phenotypic fitness was maintained at the maximum level, but embryos evolved to value structural genes over the competency gene. Over time, selection ensured that the genotype improved to a stage where competency became redundant — the Baldwin effect. \\

We conclude that in the context of expensive competencies, selection is faced with a tradeoff between competency and the structural genome: it can either pick high competencies and bear subsequent penalties, or, it can pick low competencies and improve its structural genome. Since improving the structural genome does not bear a cost, selection prioritizes improvement of the structural genome, and over time, nullifies the effect of competency. Thus early gains based on the competency gene are later assimilated into the structural genes, paralleling what has been described previously in the context of organism-level learning.


Next, we discuss the implications of our results to the fields of developmental biology and evolutionary computation, and highlight the limitations of our model. We make it explicit that significant parts of the following chapter are borrowed from previously published work, of which I was a significant contributor of. 

==> Chapters/Chapter5.tex <==
% Chapter Template

\chapter{Discussion} % Main chapter title

\label{Chapter5} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

In this body of work, we focused on a specific and novel question: the implications, for the rate and course of evolution, of a developmental process that exhibits competency at problem solving in anatomical morphospace. We produced a minimal simulation (Figure 1) that abstracted away many biological details to focus on a simple architecture: a phenotype easily optimized by traditional genetic algorithms, and a new component: competency/intelligence of the individual cells to move based on interactions with neighboring cells, simulating a single body axis morphogenetic gradient of positional information.


\subsection{Genotypic vs. Phenotypic Fitness: Cellular Competencies and Learning}

Our approach is related to the work on the role of learning in evolution. What is similar is the emphasis on genetics as the specification for a system that will then exhibit diverse behaviors that are not themselves hardcoded in the genome. Additionally, similar is the fact that DNA, as a code for specifying protein sequences, actually cannot encode directly for behavioral repertoires any more than it can directly encode morphology. What is crucially different is that traditional approaches focus on animal-scale behavior, which requires a novel and specific mechanism to evolve, such as nervous systems wired so as to facilitate specific types of learning. In our model, there is no learning needed; moreover, our system’s competency arises from a basic property of single cells: the ability to sense their neighbors, prefer those of similar type, and migrate as needed to reduce stress based on unmet expectations (e.g., intercalary regeneration in the limb). Because cells were once themselves individual organisms and are organized into networks with homeostasis, allostasis, and homeorhesis properties, evolution is working with an agential material, which has competencies that do not need to be evolved directly (are present from the start). \\

However, it is likely that the cellular competency we examine here, and the behavioral learning that has been modeled by others, interact in ways that have evolutionary impact. For example, cellular activities can be the subject of behavior shaping by signals (implemented by evolutionarily-sculpted properties of the subcellular hardware such as signaling machinery and GRNs). In other words, much as organism-level learning enables an individual’s function to be molded by signals from conspecifics and parasites; similarly, cellular competencies open cells up to beneficial or detrimental signals from other cells in the organism itself that can control them via real-time triggers. It will be interesting in future work to understand how many results from the evolutionary learning field carry over to the evolutionary implications of competency, and how these two different aspects of the divergence of genotype from phenotype interact with each other in hybrid models that have both features.

\subsection{The Role of Cellular Competency in Evolution}

We found that providing cells with a minimal homeostatic competency to improve their position in the virtual embryo results in better performance of the evolutionary search. Populations reach better fitness values faster when cellular activity is able to make up for genetic deficiencies (Figure 2). Indeed, in mixed populations, competent individuals tend to dominate and rapidly take over (Figure 4), as long as they have a minimal level of competency and/or are present in adequate numbers (Table 2). The simulation highlighted the distinction between two properties of each individual that are often conflated or obscured in simulations that do not include an explicit competency step: genotypic vs. phenotypic fitness. \\


Indeed, biology has many examples of evolution’s attempts to gauge genomes that it cannot see directly, for example by fluctuating asymmetry and the near universal standards of sexual selection for left-right symmetrical features (which in turn is correlated with lack of genetic damage). In this system, we see that competency results in good phenotypic fitness but takes selective pressure off of genotypic fitness, which settles at a sub-optimal level (Figure 3).\\


Perhaps the most interesting aspect was the role that competency plays in exacerbating the inability of selection to evaluate the genetic material that gets passed on to subsequent generations. We observed that increases in competency made it harder and harder for selection to pick the best structural genes. Specifically, the correlation between genotypic and phenotypic fitness drops to insignificant levels very rapidly (Figure 5C). This could be expected to result in complex dynamics, because competency improves fitness of individuals but impairs the ability of the evolutionary hill-climbing search in fitness space to pick out the most elite structural genomes. Thus, we studied what happens when evolution is also allowed to control the degree of competency, which is biologically realistic since cellular capacities for sensing, computation, and action are themselves under evolutionary selection. We observed that the population drives towards picking the highest competency gene value in the population (Figure 5A), settling at a value close to 470. While this value of competency is sufficient to boost an embryo’s fitness to maximum, it is not necessary. We propose the following explanation.\\

Initially when evolution begins, the ordering of the cells is far enough from ascending order that a high competency gene value is required to create individuals with high fitness. At generation 20 or so, maximum fitness is achieved by choosing high competency gene values, and by simultaneously improving structural genome quality to 57\% genotypic fitness. After generation 20, the genotypic fitness drops to a value of 52\% and stabilizes with no further improvements. From this value of genotypic fitness, a competency value of 364 would theoretically be adequate to reach peak fitness. As a result, there is no selection pressure for evolution to always pick the highest possible competency value (i.e, a value of 480 seen in the shaded area of Figure 5A), because a value of 480 confers no additional phenotypic fitness over a value of 364. They are perceived as equal by the selection process and hence a random walk between these values would suffice. The reason we notice evolution picking values close to 480 at the end of 1000 generations could be because of a stochastic component to selection of embryos with competency gene values above 364. In our experiments, if greater than 10\% of the population have a fitness of 1.0 before selection, we pick the first 10\%. This leads to the random selection of competency genes within the range of $[364, 480]$.\\


In our models, we had to make a number of quantitative choices with respect to the evolutionary process. Thus, we checked how sensitive our conclusions were to these decisions via a hyperparameter scan: re-running the simulations with different choices for various hyperparameters (see Appendix A2.3.1). Specifically, we identified mutation probability and selection stringency as key hyperparameters which could influence the results of evolution. In an effort to probe their influence on the final competency gene value attained, we ran this experiment for 132 different combinations of mutation probability and selection stringency in the range of $[0.2, 0.8]$ and recorded the stable-competency value attained for each hyperparameter combination (Figure A1 in Appendix A2.3.1). Correlation analysis revealed that a correlation of −0.4 existed between mutation probability and stable-competency-gene-value. However, no relationship was found between selection stringency and the stable-competency-gene-value. A possible reason for this could be that after generation 20, almost every embryo in the population achieves maximum phenotypic fitness, therefore there is no difference in choosing the top 20\% of the population or the top 80\% of the population. Mutation probability on the other hand has a direct influence on changing individual fitness, which explains its moderately significant relationship with the stable-competency-gene-value.

\subsection{The Paradox of Robustness}









% Mention the implications of the genotype-phenotype disparity (refer to the first part of your notes 2, I, II)

% Discussion of the costs of learning or of any other adaptive process (check mayley 1996), talk about the cost-benefit tradeoff, mention when learning actually gets canalized (mayley 1996 result).

% While taking about cost of learning mention Perter turney 1996: who claimed that if there is no cost to learning genetic assimilation (the second step of the baldwin effect (refer to the paper), will halt)

% Talk about costs of learning and how dynamics can be changed even without the baldwin effect
  
% Talk about the lack of an external environment

% Talk about developing a new class of evolutionary algorithms

==> other-chapters/pre-registration.tex <==
\chapter{Pre-Registration Document} % Main appendix title

\label{pre-registration} % For referencing this appendix elsewhere, use \ref{AppendixA}

{\Large{\textbf{Role of Cellular Competency in Evolution}}}\\
Version 2: February 12th 2023

\section{Introduction}

The conventional view of evolution is to optimize genomes towards functional goals. This overview assumes that the relationship between the genotype and the phenotype is direct. But it is not. In real biology, genes do not code for structure and function of the organism. Developmental physiology is the control layer which separates the genotype from the phenotype; during development, organisms emerge as a result of the complex set of interactions among cells, with the anatomical order being the result of cellular activities. If one were to study the nature of these cellular activities, a clear picture emerges, one which indicates that cells are active, goal-directed entities capable of solving tasks in their own local environment. We refer to this goal-directed behavior as cellular-competency. \\

As far we know, cellular-competency during morphological development is a phenomenon largely ignored in literature. We take a preliminary step to address this issue by asking how evolutionary dynamics would change if we accounted for cellular competency during development.\\

\section{Key Research Question}

\begin{itemize}
    \item[] How does cellular competency during development affect evolution? 
\end{itemize}

\section{General Hypotheses}

\begin{itemize}
    \item[1.] Populations with competency reach morphological goals faster than populations without competency.
    
    \item[2.] Evolution prefers higher competency over lower competency.
    
    \item[3.] In a mixed population, competent individuals are selected over non-competent individuals.
    
    \item[4.] Evolution prefers to improve competency rather than the structure of an embryo.

    \item[5.] Competency helps evolutionary algorithms escape local minima.
 
\end{itemize}

\section{Methods}

\subsection{Artificial Embryogeny Model}

We will answer our research question by simulating the evolution of artificial embryos in-silico. The following sections describe the components of our framework and the evolutionary algorithm employed for evolution.

\subsection{Components and Terminology}

Each artificial embryo is defined as a one-dimensional array of fixed size initialized with random integer values. Each byte of this array is termed  a “cell” of the array, carrying a value called the “cell-value”.\\

\begin{figure}[htbp]
\includegraphics[width=7cm]{other-chapters/pre-reg-images/fig1.png} 
\centering
\caption[]{Structure of an artificial embryo} \label{pfig1}
\centering
\end{figure}


Two kinds of embryos exist in our framework: a “competent embryo” and a “hardwired embryo”. A competent embryo contains competent cells. i.e, each cell has the ability to look into its neighbors’ cell-value and act in specific ways (elaborated below). The hardwired embryo on the other hand has no such capability.\\


\begin{figure}[htbp]
\includegraphics[width=7cm]{other-chapters/pre-reg-images/fig2.png} 
\centering
\caption[]{Structure of a hardwired and a competent embryo. A competent embryo can rearrange its cells whereas a hardwired embryo cannot} \label{pfig2}
\centering
\end{figure}

We define the fitness of an embryo as the degree of order in its array. If an embryo’s array has cell-values in monotonic ascending order it has maximum fitness and if it has cell-values in random order it has least fitness.\\


\begin{figure}[htbp]
\includegraphics[width=7cm]{other-chapters/pre-reg-images/fig3.png} 
\centering
\caption[]{Fitness is based on the degree of ascending order within an embryo} \label{pfig3}
\centering
\end{figure}

A hardwired population consists of a fixed number of hardwired embryos, and a competent population consists of a fixed number of competent embryos.


\subsection{Process of Evolution}

Given the above basic components, our goal is to evolve a population of embryos to reach maximum fitness by applying an evolutionary algorithm.\\

The evolutionary algorithm is a iterative process consisting of the following steps:

\begin{itemize}
    \item[1.] Development 
    \item[2.] Selection
    \item[3.] Crossover
    \item[4.] Mutation
\end{itemize}

\subsection{Development Stage}

At the start of each iteration, embryos of a population undergo development. If a competent population is being evolved, then each embryo of this population possesses “competency”, a unique trait where each cell of the embryo’s array can “look” into its neighbor’s cell’s value, and can swap cells in order to boost fitness (i.e, swap cells in a way to increase the order of arrangement of its cells). The total number of swaps it can execute is given by an integer appended to the end of the embryo’s array called the “competency gene”. This competency gene does not take part in the cell-swapping process, but simply specifies the number of swaps that the array can execute.\\

\begin{figure}[htbp]
\includegraphics[width=7cm]{other-chapters/pre-reg-images/fig4.png} 
\centering
\caption[]{A competent embryo can sense its neighbors values and swap itself to achieve local order. The number of swaps a competent embryo can execute is encoded by a value termed the "competency gene". The competency gene is not part of the morphological structure of the embryo} \label{pfig4}
\centering
\end{figure}

On the other hand, if a hardwired population is being evolved, the embryos of this population do not possess the competency trait. Therefore their cells are not capable of swapping their values.


\subsection{Selection Stage}

Post development, the fitness of each embryo in the population is calculated. We calculate the fitness by checking the number of inversions in the array. Based on the fitness, the top 10\% of the embryos in a population are selected, the rest are discarded.


\subsection{Crossover}

To repopulate the population to its original strength, we carry out a process of cross-over, where two existing embryos (parents) are cut and one half of the first embryo is combined with the second half of the second embryo to give rise to a single child.

\subsection{Mutation}

Each embryo in the repopulated population is subject to point mutations (random change in a single cell-value) based on a probability.


\subsection{Populations for Evolution}

We plan on evolving the following populations:

\begin{itemize}
    \item[1.] A hardwired population.
    \item[2.] A competent population.
    \item[3.] A mixture population (consisting of both hardwired and competent individuals mixed in different proportions)
\end{itemize}

\subsection{Hyperparameters}

Most of the hyperparameters in our model belong to those of the evolutionary algorithm. General parameters such as population size and embryo size are determined arbitrarily. Key parameters such as mutation probability and selection stringency are chosen based on a process of hyperparameter search. We plan on publishing our hyperparameter results.\\

We believe that our minimalist framework is the best way to assess the role of competency. Inclusion of realistic developmental parts would interfere with the process of competency thereby providing us a muddled view of competency’s role in evolution.

\subsection{Input Data}

The embryogeny model involves evolving a population of one-dimensional arrays. Arrays are initialized with random cell-values using a random seed generator at the start of evolution.

\subsection{Measures (Output)}

Fitness values, cell-values, and competency-gene values at every generation will be recorded.


\subsection{Analyses}

Our goal is to compare each population to every other population by plotting fitness trends, comparing cell-values, or comparing competency-gene values. \\

\textbf{Plot comparisons}: The fitness of the best embryo in each generation is plot. We confirm differences between populations visually and statistically. To confirm these differences statistically, we identify the top 3 generations with the greatest variance, and carry out a t-test at each of them.\\

\textbf{Competency-gene value comparison}: We plot the competency-gene value of the best individual and check to see how evolution picks these values. For instance, does it pick lower values, higher values, or is it chaotic with no pattern whatsoever?


\subsection{Interpretation}

If the fitness graph of the competent population is above that of the hardwired population, it indicates the advantage of competency.\\

If the competency-gene value increases over the course of evolution, it implies that evolution prefers to increase competency.\\

If the competency-gene is updated more often than any other cell-value then it implies that evolution prefers to improve competency rather than the embryo’s structure.



